Novel Aspects of IEEE SA P3109 Arithmetic Formats for Machine Learning

The IEEE P3109 draft standard defines a parameterized family of binary floating-point formats and associated operations, with a focus on facilitating machine learning. These formats allow efficient and consistent representation of values in a small number of bits. The defined formats are parameterized over width and precision in bits, signedness, and the presence of infinities. Operations are defined by decoding floating-point values to the set of closed extended reals: the reals augmented with positive and negative infinity and NaN (Not a Number). Explicit treatment of NaN and infinite operands ensures that only real arithmetic is invoked in operation definitions. Extensive rounding and saturation modes are defined; stochastic rounding is included. Operations are exception-free, accelerating throughput, with exceptional situations communicated through return values, e.g., NaN. Operations on blocks of values sharing a common scale factor are defined in terms of the underlying operations in a uniform manner. System vendors may describe approximate implementations via a novel scale-invariant measure, akin to units in the last place. Standard function definitions and various other properties are mechanically verified and generated using formal specifications.

==> wDivide.tex <==
\noindent\Case{\wDivide(\NaN, \any) \gives  \NaN}\\
\Case{\wDivide(\any, \NaN) \gives  \NaN}\\
\Case{\wDivide(+\infty, \pm\infty) \gives  \NaN}\\
\Case{\wDivide(-\infty, \pm\infty) \gives  \NaN}\\
\Case{\wDivide(\any, \zero) \gives  \NaN}\\
\Case{\wDivide(+\infty, Y) ~\If Y > \zero\gives  +\infty}\\
\Case{\wDivide(+\infty, Y) ~\If Y < \zero\gives  -\infty}\\
\Case{\wDivide(-\infty, Y) ~\If Y > \zero\gives  -\infty}\\
\Case{\wDivide(-\infty, Y) ~\If Y < \zero\gives  +\infty}\\
\Case{\wDivide(\any, \pm\infty) \gives  \zero}\\
\Case{\wDivide(X, Y) \gives X / Y}\\

